Near-Memory Computing: Past, Present, and Future

The conventional approach of moving data to the CPU for computation has become a significant performance bottleneck for emerging scale-out data-intensive applications due to their limited data reuse. At the same time, the advancement in 3D integration technologies has made the decade-old concept of coupling compute units close to the memory --- called near-memory computing (NMC) --- more viable. Processing right at the "home" of data can significantly diminish the data movement problem of data-intensive applications. In this paper, we survey the prior art on NMC across various dimensions (architecture, applications, tools, etc.) and identify the key challenges and open issues with future research directions. We also provide a glimpse of our approach to near-memory computing that includes i) NMC specific microarchitecture independent application characterization ii) a compiler framework to offload the NMC kernels on our target NMC platform and iii) an analytical model to evaluate the potential of NMC.

==> sections/cim.tex <==
\begin{figure} [!b]
\centering
\includegraphics[scale=0.7]{img/cim-3d.eps}
\caption{Computation-in-memory architecture
\label{fig:cim}}
\end{figure}

In this section, we provide a brief overview of computation-in-memory (CIM). We limit our discussion to CIM based on memristors~\cite{1083337} as they are one of the most promising candidates for the next generation of non-volatile memories. Memristors have a large resistance ratio ($R_{off}/R_{on}$), and a small write power consumption. These devices could be used both for single-level and multi-level memories. A broad range of memristor-based logic designs have been proposed:
\begin{itemize} 
    \item Boolean logic (OR, AND, NOR, etc.) ~\cite{6895258,7357122,6331426,Snider2005}
    \item Implication logic (stateful logic, complementary logic, etc.) ~\cite{statefullogic,6617731,0957-4484-23-30-305205}
    \item Threshold/majority (hybrid current mirror logic, etc.) ~\cite{6058571,6415280}
\end{itemize}

  CIM is one of the most important use-case for the memristors. Figure~\ref{fig:cim} demonstrates the concept of CIM. Essentially, integrating logic and memory at the same physical location is referred to as CIM. Usually, a crossbar architecture is used where at each junction a memristor device is placed. CMOS circuitry is used to handle the overall communication and control. 
  In literature, the first presented work is the MPU (memory processing unit)~\cite{7568648} which demonstrated the elimination of data transfer to and from the memory since the logic operations can be executed simultaneously. Therefore, this architecture can provide an order of magnitude improvement in both performance and energy efficiency. In another work, Hamdioui et al.~\cite{Hamdioui:2015:MBC:2757012.2757210} demonstrate the applicability of CIM in reducing the bottleneck of big-data computation and shows a significant reduction in energy. CIM has a lot of research potential and in the coming decade could be the next computing paradigm.
  
   However, memristors suffer from poor endurance. This issue limits the applicability to workloads with more read operations than write.  To reduce these issues exhibited by memristors Xie et al.~\cite{7987515} use a new logic design called scouting logic in which they do computation in periphery of the design.  









